Consistent Query Answering for Existential Rules with Closed Predicates

Consistent Query Answering (CQA) is an inconsistency-tolerant approach to data access in knowledge bases and databases. The goal of CQA is to provide meaningful (consistent) answers to queries even in the presence of inconsistent information, e.g. a database whose data conflict with meta-data (typically the database integrity constraints). The semantics of CQA is based on the notion of repair, that is, a consistent version of the initial, inconsistent database that is obtained through minimal modifications. We study CQA in databases with data dependencies expressed by existential rules. More specifically, we focus on the broad class of disjunctive embedded dependencies with inequalities (DEDs), which extend both tuple-generating dependencies and equality-generated dependencies. We first focus on the case when the database predicates are closed, i.e. the database is assumed to have complete knowledge about such predicates, thus no tuple addition is possible to repair the database. In such a scenario, we provide a detailed analysis of the data complexity of CQA and associated tasks (repair checking) under different semantics (AR and IAR) and for different classes of existential rules. In particular, we consider the classes of acyclic, linear, full, sticky and guarded DEDs, and their combinations.

==> 10-ocs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Open-closed-separable dependencies}
\label{sec:ocs}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We say that a dependency $\tau$ is:
\begin{itemize}\itemsep0em
    \item a \emph{closed-head} dependency if no open predicate occurs in $\head(\tau)$;
    \item an \emph{open-head} dependency if all the atoms occurring in $\head(\tau)$ are atoms with an open predicate.
\end{itemize}
Given a set of dependencies $\Sigma$, we denote by $\Sigma_c$ (resp., $\Sigma_o$) the set of closed-head (resp., open-head) dependencies occurring in $\Sigma$.

% We say that a dependency $\tau$ is a \emph{closed-head} dependency if no open predicate occurs in $\head(\tau)$. Given a set of dependencies $\Sigma$, we denote by $\Sigma_c$ the set of closed-head dependencies occurring in $\Sigma$.

% We say that a dependency $\tau$ is an \emph{open-head} dependency if all the atoms occurring in $\head(\tau)$ are atoms with an open predicate. Given a set of dependencies $\Sigma$, we denote by $\Sigma_o$ the set of open-head dependencies occurring in $\Sigma$.

In the rest of this section, we consider sets of dependencies $\Sigma$ where every $\tau\in\Sigma$ is such that, if an open predicate occurs in the head of $\tau$, then $\tau$ is non-disjunctive
and no inequality occurs in it.\footnote{This assumption is necessary in order to make our framework coincide with the one studied in~\shortcite{LMMMPS22} in the case when there are no closed predicates.}
% \nb{Questa assunzione sulle $\neq$ potrebbe essere tolta nel caso OCS, mentre è necessaria per lo splitting delle dipendenze ``miste'' generali descritto subito dopo.}
% \nb{Vogliamo motivare questa assunzione rifacendoci alle classi di existential rules considerate in~\shortcite{LMMMPS22}?\\Ric: Collegato a questo c'è l'impatto delle disuguaglianze nel body sulla complessità (perché con $\neq$ posso esprimere denial corrsipondenti a EGD).}
Under this assumption, every set of dependencies $\Sigma$ can be equivalently (w.r.t.\ the entailment task studied in this paper) transformed into a set of dependencies $\Sigma'$ such that $\Sigma'=\Sigma_o'\cup\Sigma_c'$. In other words, all the dependencies having a ``mixed'' head can be split into dependencies without mixed heads.
%%
For example, given a dependency $\tau=\forall\vseq{x}(\cnj(\vseq{x})\ra\exists y,z,w\, (P_o(y,z)\land P_c(z,w)))$, where $\cnj(\vseq{x})$ is any conjunction of atoms, $P_o\in\S_o$ and $P_c\in\S_c$, then $\tau$ is equivalent to the following set of dependencies:
\[
\begin{array}{r@{\,}l}
     \forall \vseq{x} & (\cnj(\vseq{x}) \ra \exists y,z,w\, O^\aux(y,z,w)) \\
     \forall y,z,w & (O^\aux(y,z,w)) \ra P_o(y,z)\\
     \forall y,z,w & (O^\aux(y,z,w)) \ra P_c(z,w)
\end{array}
\]
where $O^\aux$ is a fresh open predicate.

% The only dependencies that cannot be split are the ones containing both open predicates and inequalities in the head involving existential variables: e.g.\ the dependency $r(x)\rightarrow \exists y s(x,y) \wedge x\neq y$ (assuming that $s$ is an open predicate).

As usual, in the following we call \emph{frontier variables} of a dependency $\tau$ all the variables occurring both in the body and in the head of $\tau$.
Moreover, we define the set of \emph{existential positions} of a set of dependencies $\Sigma$ as the minimal set $\P$ of positions of open predicates occurring in $\Sigma$ such that:
\begin{itemize}
\item
if there exists $\tau\in\Sigma_o$ such that there is an atom with predicate $p$ in $\head(\tau)$ whose $i$-th argument is an existential head variable, then $p[i]\in\P$;
\item
if there exists $\tau\in\Sigma_o$ such that there is a frontier variable $x$ of $\tau$ only occurring in existential positions in $\body(\tau)$ and occurring in the $i$-th position of an atom with predicate $p$ in $\head(\tau)$, then $p[i]\in\P$.
\end{itemize}
%
Every position of predicates occurring in $\Sigma$ that is not an existential position of $\Sigma$ is called a \emph{non-existential position} of $\Sigma$.
%
Furthermore, we say that a variable occurring in a dependency $\tau\in\Sigma$ is \emph{grounded} in $(\tau,\Sigma)$ if it occurs in $\body(\tau)$ in at least one non-existential position of $\Sigma$.

\begin{definition}[OCS]
\label{def:ocs}
    Given a set $\Sigma$ of dependencies, we say that $\Sigma$ is \emph{open-closed-separable (OCS)} if, for every $\tau\in\Sigma_c$, all the frontier variables of $\tau$ 
    %%
    and all the variables occurring in inequality atoms in $\body(\tau)$
    %%
    are grounded in $(\tau,\Sigma)$.
    %If $\Sigma$ is OCS, we also say that $\Sigma_c$ is \emph{OCS with respect to} $\Sigma_o$.
\end{definition}

It is easy to verify that a non-existential position is a position in which, for every database $\D$, no labeled null can occur in $\chase(\D,\Sigma_o)$. Informally, this property implies a ``controlled'' interaction between $\Sigma_c$ and $\Sigma_o$ when $\Sigma$ is OCS: in particular, the dependencies in $\Sigma_c$ have effect on the OC-consistency of $\SD$, but they have no effect on OC-entailment in the case when $\D$ is OC-consistent with $\Sigma$.
%%
Moreover, when $\Sigma$ is OCS, checking the consistency of $\SD$ can be done by ``separating'' reasoning over $\Sigma_c$ and $\Sigma_o$ (see Lemma~\ref{lem:inconsistent-ocs} below). 

\begin{example}
    Let us consider again the setting illustrated in Example~\ref{ex:intro-mixed}. It is straightforward to verify that the described set of dependencies (let us indicate it with $\Sigma$) is OCS.
    In particular, the only existential position in $\Sigma$ is the second argument of the open predicate $F$, and in the second dependency (let us call it $\tau_2$) the variable $c$ occurring in such a position is not grounded in $(\tau_2,\Sigma)$. Nevertheless, $c$ is not a frontier variable of $\tau_2$ and it does not participate in any inequality of the body of $\tau_2$. 
    \qedexample
\end{example}

The following property shows that OC-entailment coincides with both open and closed entailment in the case of OC-consistent databases.

\begin{proposition}
\label{pro:entailment-consistent-ocs}
    Let $\Sigma$ be a set of OCS dependencies, let $\D$ be a database such that $\D$ is OC-consistent with $\Sigma$, and let $q$ be a BUCQ. Then, $\SD\modelsoc q$ iff $\SD\modelsopen q$ iff $\tup{\Sigma_o,\D}\modelsopen q$.% \nb{Questo lemma non viene usato da nessuna parte.}
\end{proposition}
\begin{proof}
    % It is immediate to verify that $\chase(\D,\Sigma)$\nb{la funzione $\chase$ non è stata definita per dipendenze disgiuntive} produces a canonical model for the OC-models of $\SD$. This implies that $\SD\modelsoc q$ iff $\SD\modelsopen q$. Moreover, since $\SD$ is consistent\nb{qui cosa si intende per ``consistent''?}, no dependency from $\Sigma_c$ activates the chase rule, consequently $\chase(\D,\Sigma)=\chase(\D,\Sigma_o)$, which implies that $\SD\modelsopen q$ iff  $\tup{\Sigma_o,\D}\modelsopen q$.   
    By definition, $\SD\modelsoc q$ iff $q$ evaluates to true in all the OC-models of $\SD$. Anyway, every such OC-model $\D'$ (at least one of which must exist, by the OC-consistency hypothesis) is such that $\D'_c=\D_c$, which implies that it can be computed by only chasing $\D$ w.r.t.\ $\Sigma_o$ and replace with suitable constants all the existential variables occurring in the heads of the applied rules.
    Therefore, we have that $\chase(\D,\Sigma_o)$ produces a canonical model for the OC-models of $\SD$.
    Thus, $\SD\modelsoc q$ iff $q$ evaluates to true in $\chase(\D,\Sigma_o)$, which, by Proposition~\ref{pro:chase}, is true iff $\tup{\Sigma_o,\D}\modelsopen q$.

    Now note that, for every set of facts $\D'$ whose Herbrand interpretation is a model of the FO theory $\Sigma\cup\D$, there exists an OC-model $\D''$ of $\SD$ such that $\D'\supseteq\D''$. For obtaining such $\D''$ it is indeed sufficient to remove from $\D'$ all the facts over $\S_c$ that do not belong to $\D_c$.
    Therefore, if $\SD\modelsoc q$, i.e.\ $q$ evaluates to true in each OC-model of $\SD$, then a fortiori (by monotonicity of BUCQ evaluation) it evaluates to true in each such $\D'$ (i.e.\ $\SD\modelso q$).
    %%
    On the other direction, we have that $\SD\modelso q$ clearly implies $\SD\modelsoc q$, which proves the thesis.
\end{proof}

% \medskip

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Complexity results for OCS dependencies}
% \label{sec:complexity-ocs}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the remaining part of this section, we study the data complexity of CQA for OCS dependencies. More precisely, we first consider the problem of OC-entailment, then repair checking, and finally both AR-entailment and IAR-entailment.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{OC-entailment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The set of \emph{open models} of $\tup{\Sigma,\D}$ is the set of models of $\tup{\Sigma,\D}$ when we interpret all predicates as open predicates.

% We use $\modelso$ to denote entailment with respect to the open models:  $\tup{\Sigma,\D}\modelso q$ iff $q$ is true in every open model of $\tup{\Sigma,\D}$.

% We now state the following property for OCS dependencies:

% \begin{proposition}
% \label{pro:ocs}
% Let $\Sigma$ be OCS. For every database $\D$, and for every BUCQ $q$, $\tup{\Sigma,\D}\modelsoc q$ iff $\tup{\Sigma,\D}\modelso q$.
% \end{proposition}
% \begin{proof} \nb{Da completare: sostituirebbe la seconda parte della prova della prossima proposition. Ma forse la prova successiva è più autocontenuta di questa}
% The proof follows from the fact that the standard (i.e.\ open) chase of $\tup{\Sigma,\D}$ and the ``OC-chase'' of $\tup{\Sigma,\D}$ coincide when $\Sigma$ is OCS (only constants are propagated to closed predicates), with the exception that we have to consider as inconsistent the case when a closed predicate fact outside $\D$ is generated by the chase. 
% \end{proof}

We now analyze the complexity of OC-entailment under OCS dependencies. 
% To this aim, we show the following property for such a class of dependencies.

Given an OCS set of dependencies $\Sigma$ and a dependency $\tau\in\Sigma$, let $\body_o(\tau)$ denote the CQ corresponding to the conjunction of the atoms with open predicates of $\body(\tau)$ having as existentially quantified variables all the variables 
% not occurring in other atoms of $\tau$ 
that are not grounded in $(\tau,\Sigma)$.
Similarly, $\body_c(\tau)$ denotes the (not necessarily safe) \cqineq corresponding to the conjunction of the atoms with closed predicates or inequalities of $\body(\tau)$.
% having as existentially quantified variables all the variables not occurring in other atoms of $\tau$.
%
Also, let $\groundbody(\Sigma,\D)$ denote the dependencies obtained from $\Sigma_c$ instantiating, for every $\tau\in\Sigma_c$, 
% the frontier variables and the variables occurring in inequalities in $\tau$ in the body of $\tau$
all the variables grounded in $(\tau,\Sigma)$ with constants of $\D$ in all the possible ways.
%%
Notice that, if $\tau\in\groundbody(\Sigma,\D)$, then $\body_o(\tau)$ is a BCQ, $\body_c(\tau)$ is a ground \bcqineq and $\head(\tau)$ is a \bcqineq.

\begin{lemma}
\label{lem:inconsistent-ocs}
    Let $\Sigma$ be a set of OCS dependencies.
    Then, $\D$ is OC-consistent with $\Sigma$ iff, for each $\tau\in\groundbody(\Sigma_c,\D)$,\nb{Abbiamo cambiato la def.\ di $\groundbody(\Sigma_c,\D)$ e quindi questa prova va rivista, perché va dimostrato che le extra-istanziazioni della nuova def.\ non compromettono la correttezza di questa prova.} if $\tup{\Sigma_o,\D}\modelsopen\body_o(\tau)$ and $\body_c(\tau)$ evaluates to true in $\D$, then $\head(\tau)$ evaluates to true in $\D$.
\end{lemma}
\begin{proof}
    Suppose $\D$ is OC-inconsistent with $\Sigma$. Then, it is immediate to verify that $\chase(\D,\Sigma_o)$ is inconsistent with $\Sigma_c$, which implies that there exists a dependency $\tau\in\Sigma_c$ and a substitution $\sigma$ of the variables of $\tau$ with the constants and labeled nulls occurring in $\chase(\D,\Sigma_o)$ such that $\sigma(\body(\tau))$ evaluates to true in $\chase(\D,\Sigma_o)$ and $\sigma(\head(\tau))$ evaluates to false in $\chase(\D,\Sigma_o)$.
    %%
    Now, from Definition~\ref{def:ocs} it immediately follows that there exists a substitution $\sigma$ with the above properties and such that all the frontier variables of $\tau$ and all the variables occurring in some inequality of $\body(\tau)$ are replaced by $\sigma$ with a constant. Finally, the thesis is implied by the last property and the fact that, for every BCQ $q$, $\tup{\Sigma_o,\D}\modelsopen q$ iff $q$ evaluates to true in $\chase(\D,\Sigma_o)$.
    
    The other direction of the proof is trivial.
\end{proof}

From the above two lemmas, we can establish the following complexity results.

\begin{proposition}
\label{pro:oc-ent-ocs}
    Let $\Sigma$ be a set of OCS dependencies. OC-entailment of BUCQs is:
    \begin{itemize}\itemsep0em
        \item[$(i)$] in $\aczero$ with respect to data complexity in case the dependencies of $\Sigma_o$ are either acyclic, or linear, or sticky;
        %%
        \item[$(ii)$] $\PTIME$-complete with respect to data complexity in case the dependencies of $\Sigma_o$ are either full or guarded.
    \end{itemize}
\end{proposition}
\begin{proof}
    The known \PTIME\ results for data complexity of BCQ entailment under OWA~\cite{CGL12} imply both the lower bound and, along with Lemma~\ref{lem:inconsistent-ocs}, the upper bound for the cases when $\Sigma_o$ is either guarded or full are in \PTIME.
    
    Now, suppose $\Sigma$ is OCS and $\Sigma_o$ is either acyclic, or linear, or sticky. For each of these cases it is well-known~\shortcite{CGL12,CGP12} that conjunctive query answering is first-order rewritable, i.e.\ there exists a query rewriting algorithm $\forewrite$ that, given a BUCQ $q$ and $\Sigma_o$, returns an FO sentence $\phi$ such that, for every database $\D$, $\tup{\Sigma_o,\D}\modelsopen q$ iff $\phi$ evaluates to true in $\D$.
    %%
    This immediately implies that $\D$ is OC-consistent with $\Sigma$ iff the following sentence $\consistentoc(\Sigma)$ evaluates to true in $\D$:
    \[
        \consistentoc(\Sigma)=\bigwedge_{\tau\in\Sigma_c}\forall \vseq{x} \,\big((\forewrite(\body_o(\tau)(\vseq{x}_1),\Sigma_o)\wedge\body_c(\tau)(\vseq{x}_2))\rightarrow\head(\tau)(\vseq{x}_3)\big) ,
    \]
    where $\vseq{x}_1$ are the free variables of $\body_o(\tau)$, $\vseq{x}_2$ are the free variables of $\body_c(\tau)$, $\vseq{x}_3$ are the frontier variables of $\tau$, $\vseq{x}=\vseq{x}_1\cup \vseq{x}_2$ are the variables grounded in $(\tau,\Sigma)$ (thus $\vseq{x}_3\subseteq\vseq{x})$, and $\forewrite(\body_o(\tau)(\vseq{x}_1),\Sigma_o)$ denotes the FO formula returned by the algorithm $\forewrite$ executed on the CQ $\body_o(\tau)(\vseq{x}_1)$ with respect to the dependencies $\Sigma_o$.
    This shows, together with Lemma~\ref{lem:inconsistent-ocs}, that the cases when $\Sigma_o$ is either acyclic, or linear, or sticky are in $\aczero$.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Repair checking}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As for repair checking, we start considering the case when $\Sigma_c$ is a set of denials. For this case, the following property holds.

\begin{lemma}
\label{lem:rc-denial}
    Let $\Sigma$ be a set of OCS dependencies such that $\Sigma_c$ is a set of denials. Then, for every database $\D$ and for every database $\D'$, $\D'$ is a repair of $\SD$ iff the following conditions hold:
    \begin{enumerate}\itemsep0em
        \item $\D'\subseteq\D$;
        \item $\D'$ is OC-consistent with $\Sigma$;
        \item for every atom $\alpha\in\D\setminus\D'$, $\D'\cup\{\alpha\}$ is OC-inconsistent with $\Sigma$.
    \end{enumerate}
\end{lemma}
\begin{proof}
The key point is that, if $\D'$ satisfies the above conditions, then no database $\D''$ exists such that $\D'\subset\D''\subseteq\D$ and $\D''$ is consistent with $\Sigma$. In particular, if $\D'\cup\{\alpha\}$ is OC-inconsistent, then every superset of $\D'\cup\{\alpha\}$ is guaranteed to be OC-inconsistent, because $\Sigma_c$ is a set of denials and the violation of a denial in a database implies its violation in every superset of such a database.
\end{proof}

\begin{theorem}
\label{thm:rc-denial}
    Let $\Sigma$ be a set of OCS dependencies such that $\Sigma_o$ is either guarded or full and $\Sigma_c$ is a set of denials, and let $\D$ and $\D'$ be two databases. 
    Deciding whether $\D'$ is a repair of $\SD$ is PTIME-complete in data complexity.
\end{theorem}
\begin{proof}
    First we observe that, by Lemma~\ref{lem:inconsistent-ocs} from the known data complexity of BUCQ entailment under OWA, OC-consistency can be decided in polynomial time. Therefore:
    \begin{itemize}\itemsep0em
        \item all the conditions of Lemma~\ref{lem:rc-denial} can be verified in polynomial time, which establishes the PTIME upper bound;
        \item the PTIME lower bound comes from the fact that the task of checking whether a database $\D$ is an OC-repair of $\SD$ coincides with deciding the OC-consistency of $\D$ with $\Sigma$.
    \end{itemize}
    \vspace{-1.9em}
\end{proof}

For the cases when $\Sigma$ is such that $\Sigma_c$ is a set of denials and $\Sigma_o$ is acyclic, or linear, or sticky, we define the formula $\checkrepairdenial(\Sigma_c,\Sigma_o)$ obtained by modifying the formula $\checkrepairacyclic(\Sigma)$ of Definition \ref{def:rc-sentence-acyclic} as follows:
%\footnote{The formulas $\neg\consistentprimed(\Sigma_c)$ and $\neg\consistentprimed(\Sigma,p(\vseq{x}))$ that are passed to $\ucqrewrite$ are not actually BUCQs, but it is immediate to verify that they are equivalent to BUCQs and can be easily normalized.}\nb{Lor: per controllare la consistenza, anziché passare per $\consistentprimed$ e definire $\ucqrewrite$ non potremmo usare la funzione definita poco sopra nella dimostrazione della prop.~\ref{pro:oc-ent-ocs}?}
%%
\[
\begin{array}{r@{\ }l}
\checkrepairdenial(\Sigma) =
    % & \neg\ucqrewrite(\neg\consistentprimed(\Sigma_c),\Sigma_o) \wedge \\
& \displaystyle
  \consistentocauxp(\Sigma) \wedge
     \bigwedge_{p\in\pred(\constr)}\forall \vseq{x}\,
     \Big( \big(\auxp{p}(\vseq{x})\rightarrow p(\vseq{x})\big) \wedge
     \big(p(\vseq{x}) \wedge \neg \auxp{p}(\vseq{x}) \rightarrow 
    %\ucqrewrite(\neg\consistentprimed(\Sigma,p(\vseq{x})),\Sigma_o)\big)
     \neg\consistentocauxp(\Sigma,p(\vseq{x}))\big) \Big)
\end{array}
\]
where $\vseq{x}=x_1,\ldots,x_m$ if $m$ is the arity of $p$,
%
$\consistentocauxp(\Sigma)$ denotes the formula obtained from $\consistentoc(\Sigma)$ by replacing, for every predicate $r$, every atom $r(\vseq{t})$ with $\auxp{r}(\vseq{t})$,
and $\consistentocauxp(\Sigma,p(\vseq{x}))$ denotes the formula obtained from $\consistentocauxp(\Sigma)$ by replacing every atom of the form $\auxp{p}(\vseq{t})$ (for any tuple of terms $\vseq{t})$)
%% (i.e.\ every atom whose predicate is the auxiliary version of predicate $p$)
with the subformula $(\auxp{p}(\vseq{t}) \vee \vseq{t}=\vseq{x})$.

\begin{theorem}
\label{thm:rc-ocs-acyclic-linear-sticky}
     Let $\Sigma$ be a set of OCS dependencies such that $\Sigma_c$ is a set of denials and $\Sigma_o$ is either acyclic, or linear, or sticky, and let $\D$ and $\D'$ be two databases. % such that $\D'\subseteq\D$.
    Then, the sentence $\checkrepairdenial(\Sigma)$ evaluates to true in $\D\cup\aux(\D')$ iff $\D'$ is a repair of $\SD$.
\end{theorem}
\begin{proof}
    First, it is immediate to verify that, for every instantiation $\sigma$ of $p(\vseq{x})$, the sentence $\consistentocauxp(\Sigma,\sigma(p(\vseq{x})))$ evaluates to true in $\aux(\D')$ if and only if $\consistentocauxp(\Sigma)$ evaluates to true in $\aux(\D') \cup \{\sigma(\auxp{p}(\vseq{x}))\}$.
    Then, from Lemma~\ref{lem:rc-denial} and from the fact that $\consistentocauxp(\Sigma)$ evaluates to true in $\aux(\D')$ iff $\D'$ is consistent with $\Sigma$, it follows that $\checkrepairdenial(\Sigma)$ evaluates to true in $\D\cup\aux(\D')$ iff $\D'$ is a repair of $\SD$: in particular, Condition~1 of Lemma~\ref{lem:rc-denial} is verified through the subformula $\bigwedge_{p\in\pred(\constr)}\forall \vseq{x}\,\big(\auxp{p}(\vseq{x})\rightarrow p(\vseq{x})\big)$, Condition~2 is verified through the subformula $\consistentocauxp(\Sigma)$, and Condition~3 is verified through the subformula $\bigwedge_{p\in\pred(\constr)}\forall \vseq{x}\,
     \big(p(\vseq{x}) \wedge \neg \auxp{p}(\vseq{x}) \rightarrow 
    %\ucqrewrite(\neg\consistentprimed(\Sigma,p(\vseq{x})),\Sigma_o)\big)
     \neg\consistentocauxp(\Sigma,p(\vseq{x}))\big)$.
\end{proof}

We thus obtain the following upper bound for the repair checking problem.

\begin{corollary}
\label{cor:rc-denial}
     Let $\Sigma$ be a set of OCS dependencies such that $\Sigma_c$ is a set of denials and $\Sigma_o$ is either acyclic, or linear, or sticky, and let $\D$ and $\D'$ be two databases.
     Deciding whether $\D'$ is a repair of $\SD$ is in $\aczero$ in data complexity.
\end{corollary}

Then, we establish a tight complexity result for the case in which no restriction is applied to the dependencies in $\Sigma_c$. %the dependencies in $\Sigma_o$ are either acyclic, full, guarded, linear or sticky, while the ones in $\Sigma_c$ have none of such restrictions.

\begin{theorem}
\label{thm:rc-ocs-all}
    Let $\Sigma$ be a set of OCS dependencies.
    Repair checking is coNP-complete with respect to data complexity in case the set of dependencies $\Sigma_o$ is either acyclic, or full, or guarded, or linear, or sticky.
\end{theorem}
\begin{proof}
    As for the upper bound, consider the nondeterministic procedure that decides whether $\D'$ is an OC-repair of $\SD$ by trivially applying the definition: check whether $\D'$ is OC-consistent with $\Sigma$ and there exists no $\D''$ OC-consistent with $\Sigma$ such that $\D'\subset\D''\subseteq\D$. Since Lemma~\ref{lem:inconsistent-ocs} implies that, in all the cases under examination, consistency is in \PTIME\ in data complexity, the above technique establishes a \coNP\ upper bound for the repair checking problem.
    %%
    The lower bound follows from the known \coNP-hardness of repair checking in the case when $\Sigma_o$ is empty (Theorem~\ref{thm:rc-lb-guarded-sticky}).
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\ars-entailment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As for BUCQ answering, we show that OCS dependencies enjoy the following crucial property when $\Sigma_c$ only consists of denials, which allows us to reduce both \ars- and \irs-entailment to the purely-open scenario.

\begin{lemma}
\label{lem:repairs-denials-ocs}
    Let $\Sigma$ be an OCS set of dependencies such that $\Sigma_c$ is a set of denials, and let $\D$ be a database. Then, for every BUCQ $q$, $\SD\modelsaroc q$ iff $\SD\modelsaropen q$, and $\SD\modelsiaroc q$ iff $\SD\modelsiaropen q$.
\end{lemma}
\begin{proof}
    Again, it is immediate to verify that, for every database $\D'$, $\Sigma\cup\D'$ is a consistent FO theory (under OWA) iff $\chase(\D',\Sigma)$ does not contain $\bot$ iff $\D'$ is OC-consistent with $\Sigma$. This implies that the set of repairs of $\tup{\Sigma, \D'}$ coincides with its set of OC-repairs, which in turn implies the thesis.
\end{proof}

\begin{theorem}
\label{thm:ars-denials-ocs}
    Let $\Sigma$ be an OCS set of dependencies such that $\Sigma_c$ is a set of denials, and let $\D$ be a database. Then, \ars-entailment of BUCQs is \coNP-complete with respect to data complexity when the set of dependencies $\Sigma_o$ is either acyclic, or full, or guarded, or linear or sticky.
\end{theorem}
\begin{proof}
    The proof immediately follows from Lemma~\ref{lem:repairs-denials-ocs} and from the results of~\shortcite{LMMMPS22}.\footnote{Actually, with respect to the cases studied in~\shortcite{LMMMPS22}, our language also allows for the presence of inequalities in the body of the dependencies: however, when $\Sigma$ is OCS, such inequalities only involve grounded variables, 
    %hence inequality can be easily and correctly handled considering it as an additional, generic binary predicate.
    which implies that all the upper bounds shown in~\shortcite{LMMMPS22} can be easily extended to the presence of such inequalities in the bodies of dependencies.}
\end{proof}

We also prove that, if $\Sigma_o$ is either acyclic, full, guarded, linear or sticky and none of such restrictions is applied to $\Sigma_c$, then the data complexity of \ars-entailment of BUCQs does not increase w.r.t.\ the purely-closed case.

\begin{theorem}
\label{thm:ar-ent-ocs}
    Let $\Sigma$ be a set of OCS dependencies.
    \ars-entailment of BUCQs is $\pidue$-complete with respect to data complexity in case the set of dependencies $\Sigma_o$ is either acyclic, or full, or guarded, or linear or sticky.
\end{theorem}
\begin{proof}
    First, $\SD\not\modelsaroc q$ iff there exists $\D'\subseteq\D$ such that $\D'$ is an OC-repair of $\SD$ and $\tup{\Sigma_o,\D'}\not\modelsopen q$. Now, since by Theorem~\ref{thm:rc-ocs-all} OC-repair checking is in \coNP\ in data complexity, and since $\tup{\Sigma_o,\D'}\not\modelsopen q$ can be checked in \PTIME\ in data complexity in all the cases considered, the $\pidue$ upper bound in data complexity follows.
    
    The $\pidue$ lower bound follows immediately from the fact that, in the case when $\Sigma_o$ is empty, then \ars-entailment of BUCQs coincides with \ars-entailment of BUCQs when all predicates are interpreted as closed, which implies by previously mentioned results (e.g.\ the lower bound proved in~\shortcite{CM05} for denials) that the data complexity of \ars-entailment of BUCQs (and already of instance checking) is $\pidue$-complete. 
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\irs-entailment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now consider \irs-entailment of BUCQs when $\Sigma$ is an OCS set of dependencies. As anticipated in the previous section, in the case $\Sigma_c$ only consist of denials, Lemma~\ref{lem:repairs-denials-ocs} allows us to extend the results of~\shortcite{LMMMPS22} to the scenario with open and closed predicates. In particular, if the dependencies in $\Sigma_o$ are either acyclic, linear, or sticky, then \irs-entailment is FO rewritable. 

\begin{theorem}
\label{thm:irs-denials-ocs}
    Let $\Sigma$ be an OCS set of dependencies such that $\Sigma_c$ is a set of denials, and let $\D$ be a database. Then, \irs-entailment of BUCQs is in $\aczero$ with respect to data complexity when $\Sigma_o$ is either acyclic, or linear or sticky, and is \coNP-complete with respect to data complexity when $\Sigma_o$ is either full or guarded.
\end{theorem}
\begin{proof}
    The proof immediately follows from Lemma~\ref{lem:repairs-denials-ocs} and from the results of~\shortcite{LMMMPS22}.
\end{proof}

Similarly to \ars-entailment, if $\Sigma_o$ is either acyclic, full, guarded, linear or sticky and none of such restrictions is applied to $\Sigma_c$, then the data complexity of \irs-entailment of BUCQs does not increase w.r.t.\ the purely-closed case.

\begin{theorem}
\label{thm:iar-ent-ocs}
    Let $\Sigma$ be a set of OCS dependencies.
    \irs-entailment of BUCQs is $\pidue$-complete with respect to data complexity in case the dependencies of $\Sigma_o$ are either acyclic, full, guarded, linear or sticky.
\end{theorem}
\begin{proof}
    First, we call image of a BUCQ $q$ in $\tup{\Sigma_o,\D}$ a minimal subset $M$ of $\D$ such that $\tup{\Sigma_o,M}\modelso q$.
    
    Now, consider the general nondeterministic technique described in Algorithm~\ref{alg:irs-new}.
    
    % \nb{ATTENZIONE: l'upper bound implicato da questo algoritmo è $\Sigma^p_3$ e non $\pidue$}
    % {\\\color{red} Lorenzo: Non mi è chiaro. Ad esempio con questo input ritornerebbe false:\\
    %$q=\exists x\,A(x),\quad \Sigma=\emptyset,\quad\D=\{A(1)\}$\\
    % basta prendere $M=\D'=\D''=\D$}
    % \begin{algorithm}
    % \caption{\irs-Mixed-Ent}
    % \label{alg:irs-new}
    % \begin{algorithmic}[1]
    % \REQUIRE A set of dependencies $\Sigma$, a database $\D$, a BUCQ $q$;
    % \ENSURE A Boolean value;
    % %% \STATE \textbf{let} $k$ be the maximum length of a TGD or EGD in $\Sigma$;
    % %% \STATE \textbf{let} $h$ be the number of TGDs in $\Sigma$;
    % \IF {there exists an image $M$ of $q$ in $\D$ such that
    % \\\quad there exists no $\D'\subseteq\D$ such that
    % %% \STATE \qquad $|\D'|\leq k^{h+1}$ and
    % \\\qquad $\D'$ is consistent with $\Sigma$ and
    % \\\qquad there exists $\D''$ such that 
    % \\\qquad\quad $\D'\subseteq\D''\subseteq\D$ and $\D''\cup M$ is consistent with $\Sigma$}
    % \RETURN true;
    % \ELSE\RETURN false;
    % \ENDIF
    % \end{algorithmic}
    % \end{algorithm}
    
    % \begin{algorithm}
    % \caption{\irs-Mixed-Ent}
    % \label{alg:irs-new}
    % \begin{algorithmic}[1]
    % \REQUIRE A set of dependencies $\Sigma$, a database $\D$, a BUCQ $q$;
    % \ENSURE A Boolean value;
    % %% \STATE \textbf{let} $k$ be the maximum length of a TGD or EGD in $\Sigma$;
    % %% \STATE \textbf{let} $h$ be the number of TGDs in $\Sigma$;
    % \IF {there exists $M\subseteq\D$ such that
    % \\\quad $\tup{\Sigma_o,M}\modelso q$ and
    % \\\quad there exists no $M'\subset M$ such that $q$ evaluates to true in $M'$ and
    % \\\quad there exists no $\D'\subseteq\D$ such that
    % %% \STATE \qquad $|\D'|\leq k^{h+1}$ and
    % \\\qquad $\D'$ is consistent with $\Sigma$ and
    % \\\qquad$\D'\cup M$ is recoverable from $\Sigma$}
    % \RETURN true;
    % \ELSE\RETURN false;
    % \ENDIF
    % \end{algorithmic}
    % \end{algorithm}
    
    % \begin{algorithm}
    % \caption{\irs-Mixed-Ent}
    % \label{alg:irs-new}
    % \begin{algorithmic}[1]
    % \REQUIRE A set of dependencies $\Sigma$, a database $\D$, a BUCQ $q$;
    % \ENSURE A Boolean value;
    % %% \STATE \textbf{let} $k$ be the maximum length of a TGD or EGD in $\Sigma$;
    % %% \STATE \textbf{let} $h$ be the number of TGDs in $\Sigma$;
    % \\ \STATE \textbf{let} $M_1,\ldots,M_m$ be the images of $q$ in $\tup{\Sigma_o,\D}$;
    % \\\IF {there exist $m$ subsets of $\D$ $\D_1,\ldots,\D_m$ such that
    % \\\quad every $\D_i$ is consistent with $\Sigma$ and
    % \\\quad every $\D_i\cup M_i$ is not recoverable from $\Sigma$}
    % \RETURN false;
    % \ELSE\RETURN true;
    % \ENDIF
    % \end{algorithmic}
    % \end{algorithm}
    
    % \begin{algorithm}
    % \caption{\irs-Mixed-Ent}
    % \label{alg:irs-new}
    % \begin{algorithmic}[1]
    % \REQUIRE A set of dependencies $\Sigma$, a database $\D$, a BUCQ $q$;
    % \ENSURE A Boolean value;
    % %% \STATE \textbf{let} $k$ be the maximum length of a TGD or EGD in $\Sigma$;
    % %% \STATE \textbf{let} $h$ be the number of TGDs in $\Sigma$;
    % \\ \STATE \textbf{let} $M_1,\ldots,M_m$ be the images of $q$ in $\tup{\Sigma_o,\D}$;
    % \\\IF {there exist $m$ subsets of $\D$ $\D_1,\ldots,\D_m$ such that
    % \\\quad for every i s.t.\ $1\leq i\leq m$, $\D_i$ is an OC-repair of $\SD$ and
    % \\\quad for every i s.t.\ $1\leq i\leq m$, $M_i\not\subseteq\D_i$}
    % \RETURN false;
    % \ELSE\RETURN true;
    % \ENDIF
    % \end{algorithmic}
    % \end{algorithm}
    
    \begin{algorithm}
    \caption{\irs-Mixed-Ent}
    \label{alg:irs-new}
    \begin{algorithmic}[1]
    \REQUIRE A set of dependencies $\Sigma$, a database $\D$, a BUCQ $q$;
    \ENSURE A Boolean value;
    %% \STATE \textbf{let} $k$ be the maximum length of a TGD or EGD in $\Sigma$;
    %% \STATE \textbf{let} $h$ be the number of TGDs in $\Sigma$;
    \\ \STATE \textbf{let} $M_1,\ldots,M_m$ be the images of $q$ in $\tup{\Sigma_o,\D}$;
    \\\IF {there exist $\D'$ subset of $\D$ (where $\D\setminus\D'=\{\alpha_1,\ldots,\alpha_m\}$) 
    \\\qquad and $m$ subsets $\D_1,\ldots,\D_m$ of $\D$ such that
    \\\quad for every i s.t.\ $1\leq i\leq m$, $\D_i$ is an OC-repair of $\SD$ and
    \\\quad for every i s.t.\ $1\leq i\leq m$, $\alpha_i\not\in\D_i$
    \\ and $\tup{\Sigma_o,\D}\not\modelso q$}
    \RETURN false;
    \ELSE\RETURN true;
    \ENDIF
    \end{algorithmic}
    \end{algorithm}
    
    Since repair checking in all the cases considered by the theorem is \coNP-complete in data complexity, and since for all such cases deciding whether $\tup{\Sigma_o,\D}\modelso q$ is in PTIME in data complexity, the above technique provides a $\pidue$ upper bound for the data complexity of \irs-entailment of BUCQs.
    
    %The $\pidue$ lower bound follows immediately from the fact that, in the case when $\Sigma_o$ is empty, then \irs-entailment of BUCQs coincides with \irs-entailment of BUCQs when all predicates are interpreted as closed, which implies by previously mentioned results (e.g.\ the lower bound proved in~\shortcite{CM05} for denials) that the data complexity of \irs-entailment of BUCQs (and already of instance checking) is $\pidue$-complete.
    Analogously to \ars-entailment, the $\pidue$ lower bound derives from the case when all predicates are interpreted as closed.
\end{proof}

The main complexity results for OCS dependencies established by the above properties are summarized in Table~\ref{tab:results-ocs}.

\begin{table}[t]
\centering
\setlength\tabcolsep{3pt} % riduce i margini laterali delle colonne
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{$\Sigma_o$}
& \multirow{2}{*}{$\Sigma_c$}
& \multirow{2}{*}{RC}
& BUCQ & BUCQ & BUCQ \\
& & & $\modelsoc$ & $\modelsiaroc$ & $\modelsaroc$ \\
%%
%% CLOSED = DENIALS
%%
\hline
A & D & in $\aczero$ & in $\aczero$ & in $\aczero$~\ubocs & \coNP~\ubocs \\
\hline
L & D & in $\aczero$ & in $\aczero$ & in $\aczero$~\ubocs & \coNP~\ubocs  \\
\hline
S & D & in $\aczero$ & in $\aczero$ & in $\aczero$~\ubocs & \coNP~\ubocs \\
\hline
F & D & \PTIME & \PTIME & \coNP~\ubocs & \coNP~\ubocs \\
\hline
G & D & \PTIME & \PTIME & \coNP~\ubocs & \coNP~\ubocs \\
%%
%% CLOSED = ALL
%%
\hline
A & All & \coNP & in $\aczero$ & \piduecomp & \piduecomp \\
\hline
L & All & \coNP & in $\aczero$ & \piduecomp & \piduecomp \\
\hline
S & All & \coNP & in $\aczero$ & \piduecomp & \piduecomp \\
\hline
F & All & \coNP & \PTIME & \piduecomp & \piduecomp \\
% \hline
% F & OCS (***NO, equivale al caso All***) & ?? & \PTIME & \piduecomp?? & \piduecomp \\
\hline
G & All & \coNP & \PTIME & \piduecomp & \piduecomp \\
\hline
\multicolumn{6}{c}{\small\makecell[l]{ \\[-1mm]
A = Acyclic, F = Full, G = Guarded, L = Linear,
% \smallskip 
}} \\
\multicolumn{6}{c}{\small\makecell[l]{ \\[-4mm]
S = Sticky, D = Denials
% OCS = Open-Closed-separable
\smallskip }}
\end{tabular}
%
\caption{Data complexity results for OCS sets of dependencies. All entries are completeness results, except for the $\aczero$ ones. \\\ubocsTarget these results are easily derived from~\shortcite{LMMMPS22}.}
\label{tab:results-ocs}
\end{table}

==> 3-prel.new.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% NUOVA VERSIONE CON DIPENDENZE DISGIUNTIVE
\iflong
\section{Preliminaries}
\label{sec:preliminaries}
\subsection{Databases, dependencies and queries}
\else
\section{Databases, dependencies and queries}
\label{sec:preliminaries}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iflong
\subsubsection{Syntax}
\else
\inlinesubsection{Syntax}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We call \emph{predicate signature} (or simply \emph{signature}) a set of predicate symbols with an associated arity.
%
A \emph{term} is either a variable symbol or a constant symbol.
%
A \emph{predicate atom} (or simply \emph{atom}) is an expression of the form $p(\vseq{t})$, where $p$ is a predicate of arity $n$ and $\vseq{t}$ is a $n$-tuple of terms. We say that an atom $\alpha$ is \emph{ground} (or that $\alpha$ is a \emph{fact}) if no variable occur in it.
%
An \emph{inequality atom} (or just \emph{inequality}) is an expression of the form $t\neq t'$, where $t$ and $t'$ are terms.
%
Given a first-order (FO) formula (or a set thereof) $\phi$, we denote as $\vars(\phi)$ the set of variables occurring in $\phi$.
Moreover, given an FO theory $\Phi$, we denote by $\pred(\Phi)$ the set of predicates occurring in $\Phi$.

Given a predicate signature $\S$, a \emph{DB instance} (or simply \emph{database}) $\D$ for $\S$ is a set of facts over the predicates of $\S$.
%%
Hereinafter, we assume w.l.o.g.\ that a signature always contains the special predicate $\bot$ of arity 0, and that no database contains the fact $\bot$.

\begin{definition}[CQ and BCQ]
    \label{def:cq}
    A \emph{conjunctive query with inequalities (CQ)} $q$ is an FO formula of the form $\exists \vseq{y}\, (\alpha_1\wedge\ldots\wedge\alpha_k\wedge\ineq_1\wedge\ldots\wedge\ineq_h)$, where $k\geq 0$, $h\geq 0$, $k+h\geq 1$, every $\alpha_i$ is a predicate atom, every $\ineq_i$ is an inequality, and $\vseq{y}$ is a sequence of variables each of which occurs in at least one conjunct.
    %%
    Given a CQ $\exists\vseq{y}\,(\cnj)$, we denote by $\predatoms(q)$ the set of predicate atoms occurring in $\cnj$.
    %%
    If every variable of $q$ occurs in at least one predicate atom, we say that $q$ is a \emph{safe} CQ.
    %%
    Moreover, if no variable of $q$ is free (i.e.\ all such variables occur in $\vseq{y}$), we say that $q$ is a \emph{Boolean CQ (BCQ)}.
\end{definition}

\begin{definition}[UCQ and BUCQ]
    \label{def:ucq}
    A \emph{union of conjunctive queries with inequalities (UCQ)} $q$ is an FO formula of the form
    %% \begin{equation}
    %% \label{eqn:ucq}
    $\bigvee_{i=1}^m q_i$,
    %% \end{equation}
    where $m\geq 1$ and every $q_i$ is a CQ.
    %%
    %When all such $q_i$ are BCQs, we say that $q$ is a \emph{Boolean UCQ (BUCQ)}.
    %%
    We denote by $\cq(q)$ the set of CQs occurring in $q$, i.e.\ $\cq(q)=\{q_1,\ldots,q_m\}$.
    %%
    %and we also define $\vars(q)=\bigcup_{q\in\cq(q)}\vars(q)$.
    % $\freevars(q)=\bigcup_{q\in\cq(q)}\freevars(q)$,
    % $\varsp(q)=\bigcup_{q\in\cq(q)}\varsp(q)$,
    %and $\predatoms(q)=\bigcup_{q\in\cq(q)}\predatoms(q)$. 
    %%
    If all CQs $q_i$ are safe and share the same free variables, we say that $q$ is a \emph{safe} UCQ.
    %%
    Moreover, if all CQs $q_i$ are Boolean, we say that $q$ is a \emph{Boolean UCQ (BUCQ)}.
\end{definition}

%If every variable of a CQ $q$ (resp., UCQ $q$) occur in at least one predicate atom of $\cnj$, we say that $q$ is a \emph{safe} CQ (resp., $q$ is a \emph{safe} UCQ).

Given a UCQ $q$ with free variables $\vseq{x}$, and given a tuple of constants $\vseq{t}$ of the same arity as $\vseq{x}$, we denote by $q(\vseq{t})$ the BUCQ obtained from $q$ by replacing all the occurrences of free variables with the constants in $\vseq{t}$.

We are now ready to define the notion of dependency that we use throughout the paper.\footnote{Although slightly different, Definition~\ref{def:dependency-new} is actually equivalent to the notion of disjunctive embedded dependency with inequalities \emph{and equalities} presented in~\shortcite{D18,DT05}.}

\begin{definition}[Dependency]
\label{def:dependency-new}
    Given a predicate signature $\S$, a \emph{disjunctive embedded dependency with inequalities} (\dedineq), or simply \emph{dependency}, for $\S$ is an FO sentence over the predicates of $\S$ of the form:
    \begin{equation}
    \label{eqn:dependency}
        \forall \vseq{x}\, \big(\cnj \rightarrow q \big) ,
    \end{equation}
    where $\vseq{x}$ is a sequence of variables such that $\exists \vseq{x}\,(\cnj)$ is a safe BCQ,
    and $q$ is a UCQ whose free variables occur in $\vseq{x}$,
    and such that $q(\vseq{t})$ is a safe BUCQ for any tuple $\vseq{t}$ of constants of the same arity as $\vseq{x}$.
\end{definition}

\iflong%
Given a predicate signature $\S$ and a dependency $\tau$ for $\S$ of the above
\else%
For a dependency $\tau$ of
\fi form (\ref{eqn:dependency}), we indicate with $\body(\tau)$ 
%% the formula $\alpha_1\wedge\ldots\wedge\alpha_k\wedge\ineq_1\wedge\ldots\wedge\ineq_h$, 
the CQ $\cnj$, with $\head(\tau)$ the UCQ $q=\bigvee_{i=1}^m q_i$, and with $\bodyp(\tau)$ the set $\predatoms(\cnj)$.
%% $\beta_1\wedge\ldots\wedge\beta_m\wedge\ineq_1'\wedge\ldots\wedge\ineq_\ell'$.
%% and for every $i$ such that $1\leq i\leq m$, we denote by $\headi(\tau)$ the formula $\cnj_i$, where $\econj_i(x_i)=\exists y_i\, (\cnj_i)$.
%%
%% We also denote by $\bodyp(\tau)$ the set of predicate atoms occurring in $\body(\tau)$ 
%% and denote by $\headpi(\tau)$ the set of predicate atoms occurring in $\headi(\tau)$.
%% $\{\beta_1,\ldots,\beta_m\}$.
%% We also denote by $\bodyp(\tau)$ the formula $\alpha_1\wedge\ldots\wedge\alpha_k$, and denote by $\headp(\tau)$ the formula $\beta_1\wedge\ldots\wedge\beta_m$.
%%
%% With a slight abuse of notation, we write $\alpha\in\body(\tau)$ (respectively, $\alpha\in\head(\tau)$) to denote that the atom $\alpha$ occurs in the conjunction $\body(\tau)$ (respectively, $\head(\tau)$).
%%
%% Moreover, we call \emph{frontier variables of $\tau$} the variables of $\tau$ occurring both in $\body(\tau)$ and in $\head(\tau)$. 
%
Moreover, we say that $\tau$ is \emph{non-disjunctive} if $m=1$, i.e.\ $\head(\tau)$ is a CQ, and that $\tau$ is \emph{single-head} if it is non-disjunctive and $|\predatoms(\head(\tau))|=1$.
%%
In the rest of the paper, we omit that databases and dependencies are given for a certain signature.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iflong
\subsubsection{Semantics}
\else
\inlinesubsection{Semantics}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Dependencies and safe BUCQs are subclasses of the class of domain-independent relational calculus formulas~\shortcite{AHV95}. 
%% 
Given a domain-independent sentence $\phi$ of the relational calculus and a set of facts $\D$ over the same signature, we say that $\phi$ %\emph{evaluates to true in $\D$} if the FO model isomorphic to $\D$ satisfies $\phi$.
\emph{evaluates to true (resp., to false) in $\D$}  by actually meaning that it evaluates to true (resp., to false) under the interpretation corresponding to the Herbrand model of $\D$.
%
Moreover, if $\Sigma$ is a set of dependencies, we write $\SD\modelso\phi$ if $\phi$ is satisfied by every model of the FO theory $\constr\cup\D$.\footnote{The superscript $^o$ remarks that this entailment semantics is intended under open world assumption.}
%
Given a database $\D$ and a dependency $\tau$, we say that $\tau$ is \emph{satisfied by $\D$} if $\tau$ evaluates to true in $\D$.\nb{c'è un giro contorto: "satisfies" (in FO) definisce "evaluates to true" che poi a sua volta definisce "is satisfied by", ma alla fine "satisfies" e "is satisfied by" sono in realtà la stessa cosa. Andrebbe semplificato. Vedo che Lukasiewicz non tira in ballo FOL, ma definisce solo quando un database (instance) "satisfies" una TGD o un denial (e poi usa una nozione di valutazione di una query in un database)
\\\textbf{Lor}: però la sua nozione di valutazione è data solo per CQs, mentre per le query first-order introduce comunque il concetto di modello (che per lui è un sovrainsieme del database) e quello di certain answer. Ho cercato di risolvere il cortocircuito terminologico in modo simile a come facciamo di solito (tanto l'unico altro punto in cui parliamo di modelli first-order era la Def.~\ref{def:mixed-semantics}, che ho modificato)}
%%
Given a database $\D$ and a set of dependencies $\constr$, we say that $\D$ is \emph{consistent with $\constr$} if all the dependencies of $\constr$ are satisfied by $\D$, i.e.\ if $\bigwedge_{\tau\in\Sigma}\tau$ evaluates to true in $\D$. From this definition we immediately have that:
%%
\begin{proposition}
\label{pro:consistency-ub}
    Deciding consistency of a database with a set of dependencies is in $\aczero$ \wrt data complexity.
\end{proposition}
% \begin{proof}
%     The proof immediately follows from the fact that a database $\D$ is consistent with $\Sigma$ iff $\bigwedge_{\tau\in\Sigma}\tau$ evaluates to true in $\D$, which can be done in $\aczero$ \wrt data complexity. 
% \end{proof}

Let $\D$ be a set of facts and $q=\exists \vseq{y}\,(\cnj)$ be a CQ over the same signature of $\D$.
An \emph{instantiation of $q$ in $\D$} is a substitution $\sigma$ of the variables occurring in $q$ with constants occurring in $\D$ such that 
$(i)$ $\predatoms(\sigma(\cnj))\subseteq\D$;
$(ii)$ no inequality of the form $c\neq c$ (where $c$ is a constant) occurs in $\sigma(\cnj)$. %in $\inequalities(\sigma(\cnj))$.
%%
Given a CQ $q$, an \emph{image of $q$ in $\D$} is any subset
$\{\sigma(\alpha) \mid \alpha\in\predatoms(q)\}$ of $\D$, where $\sigma$ is any instantiation of $q$ in $\D$.
Given a UCQ $q$, an \emph{image of $q$ in $\D$} is any image of $q'$ in $\D$, where $q'\in\cq(q)$.

The following property, which is immediate to verify, is implicitly leveraged throughout the work.

\begin{proposition}\label{pro:image-satisfaction}
    Given a database $\D$ and a safe BUCQ $q$, we have that $q$ evaluates to true in $\D$ iff there exists an image of $q$ in $\D$.
    %%
    Moreover, a dependency $\tau$ is satisfied by $\D$ iff, for every instantiation $\sigma$ of $\body(\tau)$ in $\D$, there exists an image of the BUCQ $\head(\sigma(\tau))$ in $\D$.
\end{proposition}

% \warn{***SONO VERAMENTE ANCORA NECESSARIE LE SEGUENTI DEFINIZIONI DI VIOLATION?? SEMBRA PROPRIO DI NO***}

% \begin{definition}[Weak violation]
% Given a set of facts $\D'$, a \emph{weak violation of $\Sigma$ in $\D'$} is a subset $\D''$ of $\D'$ such that $\D''$ is an image of the body of a dependency $\tau$ in $\Sigma$ such that, for each instantiation $\sigma$ of $\body(\tau)$ in $\D''$,
% $(i)$ $\sigma(\head(\tau))$ has no image in $\D''$ and
% $(ii)$ $\sigma(\head(\tau))$ has an image in $\D'$.
% \end{definition}

% \begin{definition}[Violation]
% Given a database $\D$ and a set of dependencies $\constr$, a \emph{violation of $\SD$} is a subset $\D'$ of $\D$ such that there exists an instantiation $\sigma$ of $\body(\tau)$ in $\D'$ such that $\sigma(\head(\tau))$ has no image in $\D$.
% \end{definition}

% \begin{proposition}
% \label{pro:consistent-violations}
%   A set of facts $\D'$ is consistent with $\Sigma$ iff $\D'$ does not contain any violation of $\tup{\Sigma,\D'}$ and does not contain any weak violation of $\Sigma$ in $\D'$.
% \end{proposition}

% \begin{proposition}
% \label{pro:recoverability-violations}
% A set of facts $\D' \subseteq \D$ is recoverable from $\SD$ iff $\D'$ does not contain any violation of $\SD$.
% \end{proposition}

% \begin{definition}[BCQ and BUCQ]\label{def:bcq}
%     A \emph{Boolean conjunctive query with inequalities (BCQ)} is an existential conjunction with no free variables, i.e.\ an FO sentence of the form:
%     \begin{equation}
%     \label{eqn:bcq}    
%     \exists \vseq{x}\, (\alpha_1\wedge\ldots\wedge\alpha_k\wedge\gamma_1\wedge\ldots\wedge\gamma_h)
%     \end{equation}
%     where every $\alpha_i$ is a predicate atom such that every variable occurring in $\alpha_i$ also occurs in $x$, and every $\gamma_i$ is an inequality on constants or variables from $x$.
%     %%
%     A \emph{Boolean union of conjunctive queries with inequalities (BUCQ)} is an FO sentence of the form $\bigvee_{i=1}^m q_i$, where each $q_i$ is a BCQ.
% \end{definition}

% We denote by $\bcq(q)$ the set of BCQs occurring in a BUCQ $q$ (i.e.\ if $\bigvee_{i=1}^m q_i$ then $\bcq(q)=\{q_1,\ldots,q_m\}$).
% %%
% Given a BCQ $q$ of the above form (\ref{eqn:bcq}) and a database $\D$, we call \emph{image of $q$ in $\D$} every image of $\alpha_1\wedge\ldots\wedge\alpha_k\wedge\gamma_1\wedge\ldots\wedge\gamma_h$ in $\D$, and given a BUCQ $q$, we call \emph{image of $q$ in $\D$} every image of every BCQ $q_i\in\bcq(q)$ in $\D$.
% %%
% Moreover, we say that $q$ \emph{has an image in $\D$} if there exists $q'\in\bcq(q)$ such that $q'$ has an image in $\D$.

%For some results presented in this paper, it is important to keep in mind that 
We point out that the images of a BCQ with $k$ predicate atoms in a set of facts $\D$ are at most $n^k$ (where $n$ is the cardinality of $\D$) and can be computed in polynomial time \wrt\ the size of the database.

%Finally, we recall the notions of model and skeptical entailment of a database and a set of dependencies under open-world assumption.

% \begin{definition}[O-model and O-entailment]
% \label{def:mixed-semantics}
%     Given a set of dependencies $\Sigma$ and two databases $\D$ and $\D'$, we say that $\D'$ is a \emph{O-model} of $\SD$ if $\D'$ is a model of the FO theory $\Sigma\cup\D$.
%     % Moreover, we say that $\D$ is \emph{O-consistent with $\Sigma$} if $\SD$ has at least one O-model.
%     Moreover, given a BUCQ $q$, we write $\SD\modelso q$ if $q$ evaluates to true in every O-model of $\SD$.
% \end{definition}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iflong
\subsection{Subclasses of dependencies}
\else
\inlinesubsection{Subclasses of dependencies}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
We say that a dependency of the form (\ref{eqn:dependency}) is \emph{linear} in the case when $|\predatoms(\cnj)|=1$.
%
Then, if $|\cq(q)|=1$ we say that the dependency is \emph{non-disjunctive}.
%
Moreover, if $|\cq(q)|=1$ and %$\vars(q)=\freevars(q)$\iflong (or, equivalently, when $\vars(q)\subseteq\vars(\cnj)$)\fi
$\vars(q)\subseteq\vars(\cnj)$, then we say that the dependency is \emph{full non-disjunctive}, or simply \emph{full}.
%
Also, we call \emph{tuple-generating dependency (TGD)} a non-disjunctive dependency having no occurrences of inequality atoms.\nb{Lor: neanche le disuguaglianze nel body?}


% Given a predicate signature $\S$, a database $\D$, and an $n$\nobreakdash-ary predicate $p$ of $\S$, we say that a set of arguments %$\Lambda$
% $a_1,\ldots,a_m$ (with $m \le n$) is a \emph{factual key} for $p$ in $\D$ if there do not exist two distinct facts $p(c_1,\ldots,c_n)$ and $p(c'_1,\ldots,c'_n)$ in $\D$ %such that $c_i=c'_i$ for each argument of $\Lambda$.\\
% whose projections \wrt $a_1,\ldots,a_m$ coincide.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%% DEFINIZIONE DI FFK / FDET
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Given a database $\D$ and a dependency $\tau$, we say that $\tau$ is \emph{forward-deterministic (\ffk) for $\D$} if, for every instantiation $\sigma$ of $\body(\tau)$ in $\D$, there exists at most one image of the BUCQ $\head(\sigma(\tau))$ in $\D$.
% %%
% Moreover, we say that a set of dependencies $\constr$ is \emph{\ffk for $\D$} if every dependency of $\Sigma$ is \ffk for $\D$.

% It is straightforward to see that non-disjunctive full dependencies are forward-deterministic independently of the database $\D$. For a set $\Sigma$ of disjunctive or non-full dependencies, deciding whether $\Sigma$ is \ffk for a database $\D$ is not a hard task.

% \begin{proposition}
% \label{pro:ffk-check}
% Deciding whether $\Sigma$ is \ffk for $\D$ is in $\aczero$ \wrt data complexity.
% \end{proposition}
% \iflong 
% \begin{proof}
% First, observe that $\Sigma$ is not \ffk for $\D$ iff there exists a dependency $\tau\in\Sigma$ and an instantiation $\sigma$ of $\body(\tau)$ in $\D$ such that there exists at least two distinct images of $\head(\sigma(\tau))$ in $\D$.
% %%
% Now let $\checkffk(\constr)$ be the following FO sentence:
% % \[
% % \begin{array}{l}
% % \displaystyle
% % \bigwedge_{\tau\in\Sigma} \forall \vseq{x}\, \big(\body(\tau) \ra \\ 
% % \displaystyle
% % \qquad
% % \bigwedge_{q\in\cq(\head(\tau))}\neg\exists \vseq{y}\,(\conj(q)\wedge\exists \vseq{y'}\,(\conj'(q)\wedge\notequal(\vseq{y},\vseq{y'})))\big)
% % \end{array}
% % \]
% \[
% \begin{array}{l}
% \displaystyle
% \bigwedge_{\tau\in\Sigma} \forall \vseq{x}\, \Big(\body(\tau) \ra \\ 
% \displaystyle
% \qquad
% \bigwedge_{q\in\cq(\head(\tau))}\forall \vseq{y}\,\big(\conj(q)\ra\forall \vseq{y'}\,(\conj'(q)\ra\equal(\vseq{y},\vseq{y'}))\big)\Big)
% \end{array}
% \]
% where:
% %%
% $x$ contains all the universally quantified variables of $\tau$;
% %%
% $y$ contains all the existentially quantified variables of $q$ (i.e.\ the variables of $q$ not appearing in $\body(\tau)$);
% %%
% $y'$ contains a copy of all the existentially quantified variables of $q$, and $\conj'(q)$ is obtained from $\conj(q)$ by replacing every variable $y_i$ from $y$ with the corresponding copy variable  $y_i'$;
% %%
% $\equal(y,y')$ is the formula
% \[
% y_1=y_1' \wedge y_2=y_2' \wedge\ldots\wedge y_m=y_m'
% \]
% % \[
% % \begin{array}{l}
% % \displaystyle
% % \bigvee_{\tau\in\Sigma} \exists \vseq{x}\, \big(\body(\tau)\wedge \exists \vseq{y}\,(\head(\tau)\wedge\exists \vseq{y'}\,(\head'(\tau)\wedge\notequal(\vseq{y},\vseq{y'})))\big)
% % \end{array}
% % \]
% % where:
% % %%
% % $x$ are all the universally quantified variables of $\tau$;
% % %%
% % $y$ are all the existentially quantified variables of $\tau$ (i.e.\ the variables appearing only in the head of $\tau$);
% % %%
% % $y'$ are a copy of all the existentially quantified variables of $\tau$, and $\head'(\tau)$ is obtained from $\head(\tau)$ by replacing every variable $y_i$ from $y$ with the corresponding copy variable  $y_i'$;
% % %%
% % $\notequal(y,y')$ is the formula
% % \[
% % (y_1\neq y_1' \vee y_2\neq y_2' \vee\ldots\vee y_m\neq y_m')
% % \]
% Now, it is immediate to verify that $\checkffk(\constr)$ evaluates to true in $\D$ iff $\constr$ is \ffk for $\D$. Consequently, the thesis follows. 
% \end{proof}
% \fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Given a set of dependencies $\constr$, we call \emph{dependency graph} of $\constr$ the directed graph $\G(\constr)$ whose vertices are the dependencies of $\constr$ and such that there is one edge from the vertex $\tau_1$ to $\tau_2$ iff the head of $\tau_1$ contains an atom whose predicate appears in a predicate atom of the body of $\tau_2$. We say that $\constr$ is \emph{acyclic} if there is no cyclic path in $\G(\constr)$.
%%
Given a set of acyclic dependencies $\constr$, we call \emph{topological order of $\constr$} any topological order of $\G(\constr)$, i.e.\ a sequence $\tup{\tau_1,\ldots,\tau_h}$ of the dependencies of $\constr$ such that, if $i\geq j$, then the vertex $\tau_i$ is not reachable from the vertex $\tau_j$ in $\G(\constr)$.

%% We call \emph{dependency graph} of $\Sigma$ the directed graph $G$ whose vertices are the predicates of $\S$ and such that there is one edge from the vertex $p_b$ to $p_h$ iff $\constr$ contains a dependency whose body (resp., head) contains an atom whose predicate is $p_b$ (resp., $p_h$). Moreover, we say that $\constr$ is \emph{acyclic}~\shortcite{AHV95} if there is no cyclic path in $G$.

We then recall the classes of guarded and sticky dependencies~\shortcite{CGL12,BLMS11,CGP12}.
%%
A dependency $\tau$ is \emph{guarded} if there exists an atom $\alpha$ of $\body(\tau)$ such that %all the variables occurring in
$\vars(\alpha) = \vars(\body(\tau))$.
%A set of dependencies is \emph{guarded} if all its dependencies are guarded.
%
Obviously, %It is immediate to verify that,
if a set of dependencies is linear, it is also guarded.
%%
As usual, in order to introduce the stickiness property, we make use of the following auxiliary \iflong inductive \fi definition. Given a set of dependencies $\constr$, for each dependency $\tau\in\constr$ we say that a variable $x$ occurring in $\body(\tau)$\footnote{We assume w.l.o.g.\ that distinct dependencies use distinct variables.} is \emph{marked} if:
\begin{itemize}\itemsep0em
    \item[$(i)$] there exists an atom of $\head(\tau)$ in which $x$ does not occur, or
    \item[$(ii)$] there exist a dependency $\tau'$ and a predicate $p$ such that $\head(\tau)$ and $\body(\tau')$ contain, respectively, $p(\vseq{t})$ and $p(\vseq{t'})$ and, for every position $i$ of $\vseq{t}$ in which $x$ occurs, the $i$-th term of $\vseq{t'}$ is a marked variable.
\end{itemize}
Then, we say that $\constr$ is \emph{sticky} if, for every dependency $\tau\in\constr$, every marked variable occurs in $\body(\tau)$ at most once.

% \begin{definition}[EGDs]\label{def:egd}
%     Given a predicate signature $\S$, an \emph{equality-generating dependency (EGD)} for $\S$ is an FO formula over the predicates of $\S$ of the form:
%     $$\forall \vseq{x}\, \alpha_1\wedge\ldots\wedge\alpha_k\wedge\gamma_1\wedge\ldots\wedge\gamma_h \rightarrow\bot$$
%     where $x$ is a vector of variables, every $\alpha_i$ (resp., $\gamma_i$) is an atom (resp., an inequality) such that every variable occurring in it also occurs in $x$.
% \end{definition}
%In the case $h=0$, an EGD is also called a \emph{denial}.
%Also comparison predicates could be added without changing the complexity results.

\medskip

\subsection{The chase}

%\nb{Ridefinire il chase}
We now recall the notion of \emph{chase} for TGDs \shortcite{FKMP05}. % for \dedsineq~\shortcite{DT05}.
Formally, given a database $\D$ and a set of TGDs $\Sigma$, we write $\chase(\D,\constr)$ for indicating the output of the following procedure. First, initialize a set of atoms $\A$ with the content of $\D$. Then, for each dependency $\tau$ in $\constr$, if there exists an instantiation $\subst$ of $\body(\tau)$ in $\D$ such that $\subst(\head(\tau))$ evaluates to false in $\D$, add to $\D$ the atoms of $\subst(\head(\tau))$, where distinct variables are replaced with fresh \emph{labelled nulls} (i.e.\ special constants that do not already occur in $\A$).
It is well-known that such a procedure may not terminate. In particular, termination is not guaranteed for cyclic and non-full sets of dependencies.

\begin{proposition}
\label{pro:chase}
    Let $\Sigma$ be a set of TGDs and let $\D$ be a database. Then, for every BUCQ $q$, $\SD\modelso q$ iff $q$ evaluates to true in $\chase(\D,\Sigma)$.\nb{Lor: Solo se $\Sigma\cup\D$ è una teoria consistente, giusto?}
\end{proposition}


\medskip

\iflong
\subsection{Complexity classes}

In this article we refer to the following computational complexity classes:
\begin{itemize}
    \item $\aczero$, i.e.\ the class of decision problems solvable by %a logspace-uniform family of circuits $\{C_n\}$, where $C_n$ has size $O(n^c)$ for some constant $c>0$ and depth $O(1)$, and gates are allowed to have unbounded fan-in
    circuit families of constant (i.e.\ independent of the input size) depth, polynomial size, and whose gates have unbounded fanin (each gate can handle and arbitrarily-large number of inputs);
    %\item NL (or NLOGSPACE), i.e.\ the class of decision problems solvable in logarithmic space by a non-deterministic Turing machine;
    \item PTIME, i.e.\ the class of decision problems solvable in polynomial time by a deterministic Turing machine;
    \item NP, i.e.\ the class of decision problems solvable in polynomial time by a non-deterministic Turing machine;
    \item coNP, i.e.\ the class of decision problems whose complement is solvable in polynomial time by a non-deterministic Turing machine;
    \item $\pidue$, i.e.\ the class of decision problems whose complement is solvable in polynomial time by a non-deterministic Turing machine augmented by an oracle for some NP-complete problem.
\end{itemize}
These classes are such that $\aczero\subseteq\text{PTIME}\subseteq\text{NP}\cup\text{coNP}\subseteq\pidue$. 
%%
Given a complexity class $C$ and a decision problem $p$, we say that $p$ is \emph{$C$-hard} if there exists a logspace reduction from every other problem in $C$ to $p$. Moreover, if $p$ does also belong to $C$, we say that $p$ is \emph{$C$-complete}.
\else
We assume the reader to be familiar with the basic notions of computational complexity. In this paper we focus on the \emph{data complexity} of the problems studied, i.e.\ the complexity with respect to the size of the database.

%For a detailed description, we refer them to the extended version of the paper.
\fi

==> tractable-closed.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{A tractable sound approximation of BUCQ Entailment under \ars and \irs Semantics}
\label{sec:tractable-closed}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\V}{\mathcal{V}}

We first show a property of repairs.

\begin{proposition}
\label{pro:repair-characterization}
    Let $\Sigma$ be a set of dependencies, let $\D$ be a database, and let $\R$ be a repair of $\SD$. Then there exist a sequence of $k$ dependencies $\tau_1,\ldots,\tau_k$, with $k\geq 0$, and a sequence $\alpha_1,\ldots,\alpha_k$ of facts such that:
    \begin{itemize}\itemsep0em
        \item[(i)] every $\tau_i$ is obtained from some $\tau\in\Sigma$ by instantiating its body variables on the constants of $\D$;
        \item[(ii)] every $\alpha_i$ occurs in $\body(\tau_i)$;
        %% \item[(iii)] $\bodyp(\tau_i)\setminus\R=\{\alpha_i\}$ (i.e.\ $\alpha_i$ is the only atom from $\body(\tau_i)$ not occurring in $\R$);
        \item[(iii)] $\bodyp(\tau_i)\subseteq\R_{i-1}$ and $\R_{i-1}\not\models\head(\tau_i)$, where $\R_0=\D$, $\R_k=\R$ and, for every $i$ such that $1\leq i\leq k$, $\R_i=\R_{i-1}\setminus\{\alpha_i\}$;
        %\item[(iv)] $\R$ is consistent with $\Sigma$.\nb{visto che non è un if and only if, questo punto a cosa serve?}
    \end{itemize}
\end{proposition}
\begin{proof}
Let $\R$ be a repair of $\SD$ and let $k=|\D\setminus\R|$. We inductively define a sequence of dependencies $\tau_1,\ldots,\tau_k$ and a sequence of facts $\alpha_1,\ldots,\alpha_k$ as follows.
%%
%% and let $\D\setminus\R=\{\alpha_1,\ldots,\alpha_k\}$. 
Let $\R_0=\D$.
For every $i$ such that $1\leq i\leq k$, since $\R\subset\R_{i-1}$, $\R_{i-1}$ is not consistent with $\Sigma$, thus there exists a dependency $\tau_i$ obtained from some $\tau\in\Sigma$ by instantiating its body variables on the constants of $\D$ and such that $\bodyp(\tau_i)\subseteq\R_{i-1}$ and $\R_{i-1}\not\models\head(\tau_i)$. Now, since $\R$ is consistent with $\Sigma$, and since $\R\subset\R_{i-1}$, it follows that $\bodyp(\tau_i)\cap\R=\emptyset$, consequently $\bodyp(\tau_i)\setminus\R\neq\emptyset$. So let $\alpha_i$ be any atom in $\bodyp(\tau_i)\setminus\R\neq\emptyset$ and let $\R_i=\R_{i-1}\setminus\{\alpha_i\}$. 
%%
It is immediate to verify that the sequence of dependencies $\tau_1,\ldots,\tau_k$ and the sequence of facts $\alpha_1,\ldots,\alpha_k$ thus defined satisfy conditions $(i)$, $(ii)$, $(iii)$, $(iv)$ of the theorem.
%%
%% It is easy to verify that there exists a sequence of dependencies $\Theta=\tau_1,\ldots,\tau_k$ and a sequence of facts $\F=\alpha_1,\ldots,\alpha_k$ as in the theorem, such that conditions (i), (ii), (iv) and (v) hold. Now, suppose that such sequences do not satisfy condition (iii). Let $\tau_i$ be a dependency violating condition (iii), i.e.\ such that $\R\setminus\bodyp(\tau_i)=\{\alpha_i,\alpha_{j_1},\ldots,\alpha_{j_h}\}$ for some $h\geq 1$. Of course, $j>i_\ell$ for every $\ell\in\{1,\ldots,h\}$(otherwise $\bodyp(\tau_i)\not\subseteq\R_{i-1}$). Now consider the sequence of dependencies $\Theta'$ obtained from $\Theta$ eliminating $\tau_i$ and the sequence of facts $\F'$ obtained from $\F$ eliminating $\alpha_i$. Clearly, such modified sequences do not satisfy conditions (v) (otherwise $\R$ would not be a repair since $\R\cup\{\alpha_i\}$ would be consistent with $\Sigma$), so there exists a $\tau'$ obtained from some $\tau\in\Sigma$ by instantiating its body variables on the constants of $\D$ such that $\bodyp(\tau')\subseteq\R\cup\{\alpha_i\}$ and $\R\cup\{\alpha_i\}\not\models\head(\tau')$. Since $\R$ is consistent with $\Sigma$, it follows that $\alpha_i$ occurs in $\body(\tau_i)$. Consequently, if $\Theta''$ is the sequence obtained adding $\tau'$ at the end of the sequence $\Theta'$ and $\F''$ is the sequence obtained adding $\alpha_i$ at the end of the sequence $\F'$, we have that $\Theta''$ and $\F''$ satisfy conditions (i), (ii), (iv), (v) of the theorem; moreover, the last elements of the sequences ($\tau'$ and $\alpha_i$) satisfy condition (iii). $\Theta''$ and $\F''$ have one less violation of condition (iii) than $\Theta$ and $\F$ (while they produce the same repair $\R$). Iterating the above argument, it is immediate to conclude that there exists a sequence of dependencies and a sequence of facts that generate $\R$ and satisfy all five conditions of the theorem.
%%
%% Conversely, suppose that $\R$ is generated by $\Theta$ and $\F$, and suppose that $\R$ is not a repair of $\SD$, i.e.\ there exists $\alpha_i$ such that $\R\cup\{\alpha_i\}$ is consistent with $\Sigma$. But now, the dependency $\tau_i$ is such that: (i) $\bodyp(\tau_i)\subseteq\R\cup\{\alpha_i\}$, since by hypothesis $\R\setminus\bodyp(\tau_i)=\{\alpha_i\}$; and (ii) $\R\cup\{\alpha_i\}\not\models\head(\tau_i)$, since $\R\cup\{\alpha_i\}\subseteq\R_i$ and by hypothesis $\R_i\not\models\head(\tau_i)$. Consequently, $\R\cup\{\alpha_i\}$ is not consistent with $\Sigma$, contradicting the hypothesis. Hence, $\R$ is a repair of $\SD$.
\end{proof}

Let $\D',\D''$ be databases and let $\V$ be a set of sets of facts.
Given a dependency $\tau$, we call \emph{violation of $\tau$ in $(\D',\D'',\V)$} any set of facts $F$ such that there exists an instantiation $\sigma$ of the variables of the body of $\tau$ such that:
\begin{itemize}[itemsep=0em,topsep=0.3em]
    \item[$(i)$] $F=\bodyp(\sigma(\tau))\subseteq\D'$;
    \item[$(ii)$] $\D''\not\models\head(\sigma(\tau))$;
    \item[$(iii)$] for every $V\in\V$, $F\not\supseteq V$.%$V\not\subseteq\bodyp(\sigma(\tau))$.
\end{itemize}
%
Moreover, for the sake of brevity we call \emph{violation of $\tau$ in $\D'$} any violation of $\tau$ in $(\D',\D',\emptyset)$.

We now define an algorithm that, given a set of dependencies $\Sigma$ and a database $\D$ and a BUCQ $q$, returns a subset of $\D$.

\begin{algorithm}
\caption{\algiarapprox}
\label{alg:iar-approx}
\begin{algorithmic}[1]
\REQUIRE A set of dependencies $\Sigma$, a database $\D$, a BUCQ $q$;
\ENSURE A Boolean value;
\STATE $\D'\gets\D$;
\REPEAT{
    \STATE $\D_{\mathit{old}}'\gets\D'$;
    \FOREACH {linear dependency $\tau\in\Sigma$}{
        \FOREACH {violation $V$ of $\tau$ in $\D'$}{
            \STATE $\D'\gets\D'\setminus V$;
        }
        \ENDFOR
    }
    \ENDFOR
}
\UNTIL {$\D'=\D_{\mathit{old}}'$;}
\STATE $\V\gets\emptyset$;
\FOREACH {dependency $\tau\in\Sigma$}{
    \FOREACH {violation $V$ of $\tau$ in $\D'$}{
        \STATE $\V\gets\V\cup \{V\}$;
    }
    \ENDFOR
}
\ENDFOR
\STATE $\D''\gets\D'\setminus (\bigcup_{V\in\V} V)$;
\REPEAT
    \STATE $\D_{\mathit{old}}''\gets\D''$;
    \FOREACH {dependency $\tau\in\Sigma$}{
        \FOREACH {violation $V$ of $\tau$ in $(\D',\D'',\V)$}{
            \STATE $\D''\gets\D''\setminus V$;
        }
        \ENDFOR
    }
    \ENDFOR
\UNTIL $\D''=\D_{\mathit{old}}''$;
\IF{$\D''\models q$}
    \RETURN true;
\ELSE\RETURN false;
\ENDIF
\end{algorithmic}
\end{algorithm}

% \begin{tabbing}
% Algorithm Approximate-IAR-Entailment \\
% Input: set of dependencies $\Sigma$, database $\D$, query $q$ \\
% Output: true or false \\
% be\=gin \\
% \> $\D'=\D$; \\
% \> re\=peat \\
% \>\> $\D_{\mathit{old}}'=\D'$; \\
% \>\> fo\=r each linear dependency $\tau\in\Sigma$ do \\
% \>\>\>  for each violation $V$ of $\tau$ in $\D'$ do $\D'=\D'\setminus V$; \\
% \> until $\D'=\D_{\mathit{old}}'$; \\
% \> $\V=\emptyset$; \\
% \> fo\=r each dependency $\tau\in\Sigma$ do \\
% \>\>  for each violation $V$ of $\tau$ in $\D'$ do $\V=\V\cup \{V\}$; \\
% \> $\D''=\D'\setminus (\bigcup_{V\in\V} V)$; \\
% \> re\=peat \\
% \>\> $\D_{\mathit{old}}''=\D''$; \\
% \>\> fo\=r each dependency $\tau\in\Sigma$ do \\
% \>\>\>  for each violation $V$ of $\tau$ in $(\D',\D'',\V)$ do $\D''=\D''\setminus V$; \\
% \> until $\D''=\D_{\mathit{old}}''$; \\
% \> if $\D''\models q$ \\
% \> then return true \\
% \> else return false \\
% end
% \end{tabbing}

\begin{lemma}
\label{lem:approx-iar}
Let $\D''$ be the database computed by \algiarapprox$(\Sigma,\D,q)$. Then, $\D''\subseteq\intrep(\D)$.
\end{lemma}
\begin{proof}
First, it is immediate to verify that $\reps(\D')=\reps(\D)$.
{\color{red} \\proposta: $$\Sigma'=\{\sigma(\tau) \mid \tau\in\Sigma\text{, $\sigma$ is an instantiation of $\body(\tau)$ in\ }\D'\}$$}
Then, let $\Sigma_g(\D')$ be the set of all the ground instantiations\nb{Nei preliminaries il termine instantiation indica a una substitution} of the body variables of the dependencies of $\Sigma$ on the constants occurring in $\Sigma\cup\D'$. Let $\Sigma'$ be the set of dependencies obtained from $\Sigma_g(\D')$ deleting all the dependencies $\tau$ such that $\D'\not\models\body(\tau)$. Of course, we have that $\repsp(\D')=\repsg(\D')$, and consequently $\repsp(\D')=\reps(\D)$.

Let now $\R\in\repsp(D')$. We prove that $\D''\subseteq\R$.
First, by Proposition \ref{pro:repair-characterization}
there exist a sequence of dependencies $\tau_1,\ldots,\tau_k$ and a sequence of facts $\alpha_1,\ldots,\alpha_k$ (for some $k\geq 0$) such that every $\tau_i\in\Sigma'$ and $\R=\R_k$, where
$\R_0=\D'$ and, for every $i$ such that $1\leq i\leq k$,
$\R_{i}=\R_{i-1}\setminus\{\alpha_i\}$, where $\alpha_i\in\bodyp(\tau_i)$, $\bodyp(\tau_i)\subseteq\R_i$ and $\R_i\not\models\head(\tau_i)$.
W.l.o.g.\ we can assume that the sequence of dependencies is such that, if $\R_0\not\models\head(\tau_i)$ and $\R_0\models\head(\tau_j)$, then $i<j$.

Now we prove by induction that $\D''\subseteq\R$ (i.e.\ every deletion done in the above construction of $\R$ is also done in the construction of $\D''$).
\begin{itemize}[itemsep=0em,topsep=0.3em]
    \item[$\lozenge$] Base case (step 1 of the construction of $\R$): suppose that $\tau_1\in\Sigma$ is such that $\bodyp(\tau_1)\in\R_0$ and $\R_0\not\models\head(\tau_1)$. Since $\R_0=\D'$, it follows that $\bodyp(\tau_1)\in\V$, and since by definition of the algorithm $\D''\cap (\bigcup_{V\in\V} V) =\emptyset$, it follows that $\D''\subseteq\R_1$.

    \item[$\lozenge$] Inductive case: suppose $\D''\subseteq \R_i$. We have that $\tau_{i+1}\in\Sigma$ is such that $\bodyp(\tau_{i+1})\in\R_i$ and $\head(\tau_{i+1})\not\in\R_i$. Therefore, $\bodyp(\tau_{i+1})\in\R_i$ and $\head(\tau_{i+1})\not\in\D''$. 
    Now, we have two cases:
    \begin{itemize}
        \item[(i)] $\R_0\not\models\head(\tau_{i+1})$. In this case, it follows that $\bodyp(\tau_{i+1})\in\V$, and since by definition of the algorithm $\D''\cap (\bigcup_{V\in\V} V) =\emptyset$, it follows that $\D''\subseteq\R_{i+1}$;
    
        \item[(ii)] $\R_0\models\head(\tau_{i+1})$. In this case, from the hypothesis that if $\R_0\not\models\head(\tau_i)$ and $\R_0\models\head(\tau_j)$, then $i<j$, it follows that $V\not\subseteq \R$ for every $V\in\V$, consequently there exists no $V\in\V$ such that $V\subset\bodyp(\tau_{i+1})$. Hence, $\tau_{i+1}=\sigma(\tau)$ for some $\tau\in\Sigma$ and $\bodyp(\sigma(\tau))$ is a violation of $\tau$ in $(\D',\D'',\V)$. Consequently, by definition of the algorithm, $\bodyp(\sigma(\tau))\cap\D''=\emptyset$, which implies that $\D''\subseteq\R_{i+1}$.
    \end{itemize}
\end{itemize}

Hence, for every repair $\R$ of $\SD$ it holds $\D''\subseteq\R$, which implies $\D''\subseteq\intrep(\D)$.
\end{proof}

The above lemma immediately implies the following property.

\begin{theorem}
\label{thm:approx-iar}
Let $\Sigma$ be a set of dependencies, let $\D$ be  database and let $q$ be a BUCQ. If \algiarapprox$(\Sigma,\D,q)$ returns true, then $\SD$ \irs-entails $q$.
\end{theorem}

Finally, it is easy to verify that the algorithm \algiarapprox$(\Sigma,\D,q)$ runs in polynomial time with respect to the size of $\D$ (in particular, observe that the number of possible instantiations of the variables of the body of a dependency $\tau$ on the constants of $\D$ is bounded by $n^k$, where $n$ is the size of $\D$ and $k$ is the size of $\tau$).


